DORIS-MAE: Scientific Document Retrieval using Multi-level Aspect-based Queries

In scientific research, the ability to effectively retrieve relevant documents based on complex, multifaceted queries is critical. Existing evaluation datasets for this task are limited, primarily due to the high cost and effort required to annotate resources that effectively represent complex queries. To address this, we propose a novel task, Scientific DOcument Retrieval using Multi-level Aspect-based quEries (DORIS-MAE), which is designed to handle the complex nature of user queries in scientific research. We developed a benchmark dataset within the field of computer science, consisting of 100 human-authored complex query cases. For each complex query, we assembled a collection of 100 relevant documents and produced annotated relevance scores for ranking them. Recognizing the significant labor of expert annotation, we also introduce Anno-GPT, a scalable framework for validating the performance of Large Language Models (LLMs) on expert-level dataset annotation tasks. LLM annotation of the DORIS-MAE dataset resulted in a 500x reduction in cost, without compromising quality. Furthermore, due to the multi-tiered structure of these complex queries, the DORIS-MAE dataset can be extended to over 4,000 sub-query test cases without requiring additional annotation. We evaluated 17 recent retrieval methods on DORIS-MAE, observing notable performance drops compared to traditional datasets. This highlights the need for better approaches to handle complex, multifaceted queries in scientific research. Our dataset and codebase are available at https://github.com/Real-Doris-Mae/Doris-Mae-Dataset.

==> candidate_pool.tex <==
\clearpage









% We also provide the percentage of changes:\\
% 36.364\%, 30.0\%, 23.077\%, 12.5\%, 11.765\%, 11.111\%, 10.0\%, 8.696\%, 8.696\%, 6.667\%, 6.25\%, 6.25\%, 5.263\%, 5.263\%, 4.762\%, 0.0\%, 0.0\%, 0.0\%, 0.0\%, 0.0\%, 0.0\%, 0.0\%, 0.0\%, 0.0\%, 0.0\%, 0.0\%, 0.0\%, -6.25\%, -6.667\%, -7.143\%, -7.692\%, -8.0\%, -8.696\%, -9.091\%, -9.524\%, -10.0\%, -10.0\%, -10.526\%, -10.714\%, -11.111\%, -12.5\%, -12.903\%, -13.793\%, -17.647\%, -17.857\%, -19.231\%, -25.0\%, -25.0\%, -27.778\%, -36.111\%.

